Selective Sequential Model Selection

Many model selection algorithms produce a path of fits specifying a sequence of increasingly complex models. Given such a sequence and the data used to produce them, we consider the problem of choosing the least complex model that is not falsified by the data. Extending the selected-model tests of Fithian et al. (2014), we construct p-values for each step in the path which account for the adaptive selection of the model path using the data. In the case of linear regression, we propose two specific tests, the max-t test for forward stepwise regression (generalizing a proposal of Buja and Brown (2014)), and the next-entry test for the lasso. These tests improve on the power of the saturated-model test of Tibshirani et al. (2014), sometimes dramatically. In addition, our framework extends beyond linear regression to a much more general class of parametric and nonparametric model selection problems. To select a model, we can feed our single-step p-values as inputs into sequential stopping rules such as those proposed by G'Sell et al. (2013) and Li and Barber (2015), achieving control of the familywise error rate or false discovery rate (FDR) as desired. The FDR-controlling rules require the null p-values to be independent of each other and of the non-null p-values, a condition not satisfied by the saturated-model p-values of Tibshirani et al. (2014). We derive intuitive and general sufficient conditions for independence, and show that our proposed constructions yield independent p-values.

==> tables/diabetes.tex <==
\begin{tabular}{|l|c|c|c|c|c|}
\hline
 Step & Variable &  Nominal pvalue &  Saturated pvalue &  MaxT pvalue \\
\hline
    1 &      bmi &            0.00 &              0.00 &         0.00 \\
    2 &      ltg &            0.00 &              0.00 &         0.00 \\
    3 &      map &            0.00 &              0.05 &         0.00 \\
    4 &  age:sex &            0.00 &              0.33 &         0.02 \\
    5 &  bmi:map &            0.00 &              0.76 &         0.07 \\
    6 &      hdl &            0.00 &              0.25 &         0.06 \\
    7 &      sex &            0.00 &              0.00 &         0.00 \\
    8 &    glu^2 &            0.02 &              0.03 &         0.37 \\
    9 &    age^2 &            0.11 &              0.55 &         0.93 \\
   10 &  map:glu &            0.17 &              0.91 &         0.92 \\
   11 &       tc &            0.15 &              0.37 &         0.22 \\
   12 &      ldl &            0.06 &              0.15 &         0.02 \\
   13 &    ltg^2 &            0.00 &              0.07 &         0.05 \\
   14 &  age:ldl &            0.19 &              0.97 &         0.84 \\
   15 &   age:tc &            0.08 &              0.15 &         0.06 \\
   16 &  sex:map &            0.18 &              0.05 &         0.39 \\
   17 &      glu &            0.23 &              0.45 &         0.56 \\
   18 &      tch &            0.31 &              0.71 &         0.81 \\
   19 &  sex:tch &            0.22 &              0.40 &         0.45 \\
   20 &  sex:bmi &            0.27 &              0.60 &         0.55 \\
\hline
\end{tabular}


==> tables/error_rates_10.tex <==

\newcommand{\guarantee}[1]{{\bf #1}}
{\small 
\begin{tabular}{|l l|cccccc|}
\hline
{} & {} &  $\P(\hk \geq k_0)$ &  $\text{FWER}$ &  $\text{cFWER}$ &  $\text{FDR}$ &  $\text{FDR}^{\text{full}}$ &  $\E[S^{\text{full}}]$ \\ \hline
Nominal & BasicStop & 0.90 & 0.82 & 0.92 & 0.245 & 0.331 & 6.89 \\ 
Nominal & ForwardStop & 0.96 & 0.95 & 0.99 & 0.520 & 0.596 & 6.96 \\ 
Max-z & BasicStop & 0.47 & \guarantee{0.04} & \guarantee{0.09} & \guarantee{0.006} & 0.053 & 6.32 \\ 
Max-z & ForwardStop & 0.77 & 0.39 & 0.50 & \guarantee{0.068} & 0.137 & 6.74 \\ 
Max-t & BasicStop & 0.45 & \guarantee{0.05} & \guarantee{0.11} & \guarantee{0.006} & 0.051 & 6.24 \\ 
Max-t & ForwardStop & 0.75 & 0.34 & 0.45 & \guarantee{0.059} & 0.125 & 6.70 \\ 
Saturated & BasicStop & 0.01 & 0.00 & 0.00 & 0.000 & 0.027 & 2.51 \\ 
Saturated & ForwardStop & 0.15 & 0.03 & 0.21 & 0.004 & 0.038 & 3.72 \\ 
Knockoff & & 0.36 & --- & --- & --- & 0.142 & 4.55 \\ 
Knockoff+ & & 0.07 & --- & --- & --- & \guarantee{0.028} & 0.52 \\  \hline
\end{tabular}}
